An efficient estimator of the parameters of the Generalized Lambda Distribution

Estimation of the four generalized lambda distribution parameters is not straightforward, and available estimators that perform best have large computation times. In this paper, we introduce a simple two-step estimator of the parameters that is comparatively very quick to compute and performs well when compared with other methods. This computational efficiency makes the use of bootstrapping to obtain interval estimators for the parameters possible. Simulations are used to assess the performance of the new estimators and applications to several data sets are included.

==> CoverageSkew.tex <==
\begin{table}
\footnotesize
 \centering
\caption{This table shows the coverage probability (cp), mean width ($\Bar{\omega}$) and median width (m) of bootstrap confidence intervals for the l3-l4 of the closest GLD distribution. These values are obtained using 500 bootstrap re samples and 500 iterations}
\begin{tabular}{ccccccc@{\hskip 0.35in}cccc@{\hskip 0.35in}cccc@{\hskip 0.35in}cccc}
\toprule
\textit{n} & \textit{F} && \multicolumn{4}{c}{Cauchy-QOR} & \multicolumn{4}{c}{Lognormal-QOR} & \multicolumn{4}{c}{TM} & \multicolumn{4}{c}{PM}\\
 &  & &norm & basic & perc & bca & norm & basic & perc & bca & norm & basic & perc & bca & norm & basic & perc & bca\\
 \midrule
100 & Normal & cp & 1 & 1 & 1 & 0.994 & 1 & 1 & 1 & 0.992 & 0.982 & 0.978 & 0.954 & 0.97 & 0.986 & 0.988 & 0.99 & 0.966\\
& &$\Bar{\omega}$ & 106.3 & 168.4 & 168.4 & 132.1 & 106.4 & 168.4 & 168.4 & 135.3 & 0.495 & 0.487 & 0.487 & 0.484 & 1.551 & 1.656 & 1.656 & 1.683\\
&  & m & 105.8 & 223.4 & 223.4 & 112.6 & 105.8 & 223.3 & 223.3 & 112.6 & 0.466 & 0.470 & 0.470 & 0.471 & 1.472 & 1.606 & 1.606 & 1.675\\
\cmidrule{2-19}
 &$\chi^2_5$ & cp & 1 & 1 & 0.998 & 0.996 & 1 & 1 & 1 & 0.998 & 0.982 & 0.962 & 0.958 & 0.974 & 0.888 & 0.872 & 0.994 & 0.916\\
& &$\Bar{\omega}$ & 108.1 & 166.9 & 166.9 & 126.1 & 108.6 & 167.5 & 167.5 & 135.6 & 1.021 & 0.857 & 0.857 & 0.707 & 1.925 & 1.903 & 1.903 & 1.837\\
&  & m & 106.2 & 166.0 & 166.0 & 113.8 & 107.1 & 166.1 & 166.1 & 113.9 & 0.798 & 0.638 & 0.638 & 0.600 & 1.987 & 1.967 & 1.967 & 1.884\\
\cmidrule{2-19}
& Lognormal & cp & 1 & 1 & 0.996 & 0.98 & 1 & 0.998 & 0.994 & 0.984 & 0.980 & 0.952 & 0.950 & 0.948 & 0.758 & 0.678 & 0.992 & 0.810\\
& &$\Bar{\omega}$ & 109.3 & 166.9 & 166.9 & 123.4 & 110.2 & 168.1 & 168.1 & 127.2 & 2.378 & 2.088 & 2.088 & 1.542 & 2.745 & 2.551 & 2.551 & 2.351\\
&  & m & 107.9 & 171.5 & 171.5 & 115.6 & 108.7 & 183.3 & 183.3 & 115.7 & 2.190 & 1.664 & 1.664 & 1.040 & 2.792 & 2.565 & 2.565 & 2.422\\
\cmidrule{2-19}
& Beta & cp & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0.992 & 0.986 & 0.96 & 0.98 & 0.962 & 0.952 & 0.986 & 0.928\\
& &$\Bar{\omega}$ & 106.2 & 163.9 & 163.9 & 130.2 & 106.7 & 165.3 & 165.3 & 133.6 & 0.902 & 0.731 & 0.731 & 0.645 & 1.829 & 1.919 & 1.919 & 1.909\\
&  & m & 105.5 & 164.4 & 164.4 & 113.2 & 105.6 & 164.6 & 164.6 & 112.9 & 0.671 & 0.577 & 0.577 & 0.562 & 1.797 & 1.929 & 1.929 & 1.909\\
\midrule
250 & Normal & cp & 1 & 0.988 & 0.986 & 0.984 & 1 & 0.814 & 0.832 & 0.858 & 0.946 & 0.948 & 0.95 & 0.946 & 0.972 & 0.98 & 0.966 & 0.944\\
& &$\Bar{\omega}$ & 82.53 & 0.447 & 0.447 & 11.44 & 82.34 & 0.429 & 0.429& 9.209 & 0.252 & 0.256 & 0.256 & 0.256 & 0.748 & 0.766 & 0.766 & 0.796\\
&  & m & 85.39 & 0.400 & 0.400 & 0.405 & 79.35 & 0.377 & 0.377 & 0.383 & 0.249 & 0.252 & 0.252 & 0.252 & 0.693 & 0.694 & 0.694 & 0.712\\
\cmidrule{2-19}
 &$\chi^2_5$ & cp & 1 & 0.978 & 0.976 & 0.988 & 1 & 0.972 & 0.984 & 0.984 & 0.962 & 0.954 & 0.958 & 0.956 & 0.964 & 0.938 & 0.984 & 0.948\\
& &$\Bar{\omega}$ & 83.03 & 3.011 & 3.011 & 56.78 & 82.64 & 2.386 & 2.386 & 19.313 & 0.301 & 0.304 & 0.304 & 0.302 & 1.195 & 1.218 & 1.218 & 1.170\\
&  & m & 86.73 & 0.515 & 0.515 & 0.529 & 86.72 & 0.462 & 0.462 & 0.456 & 0.296 & 0.302 & 0.302 & 0.297 & 1.166 & 1.276 & 1.276 & 1.169\\
\cmidrule{2-19}
& Lognormal & cp & 1 & 0.992 & 0.892 & 0.966 & 1 & 0.986 & 0.908 & 0.964 & 0.982 & 0.972 & 0.952 & 0.964 & 0.862 & 0.794 & 0.978 & 0.872\\
& &$\Bar{\omega}$ & 89.35 & 11.38 & 11.38 & 127.2 & 87.94 & 9.312 & 9.312 & 68.69 & 1.032 & 0.774 & 0.774 & 0.588 & 2.173 & 2.000 & 2.000 & 1.8874\\
&  & m & 86.84 & 1.111 & 1.111 & 204.1 & 86.47 & 0.891 & 0.891 & 0.965 & 0.563 & 0.502 & 0.502 & 0.484 & 2.277 & 2.107 & 2.107 & 2.034\\
\cmidrule{2-19}
& Beta & cp & 1 & 0.992 & 0.982 & 0.994 & 1 & 0.986 & 0.994 & 0.994 & 0.978 & 0.976 & 0.968 & 0.968 & 0.978 & 0.98 & 0.958 & 0.942\\
& &$\Bar{\omega}$ & 82.17 & 2.415 & 2.415 & 31.45 & 82.13 & 2.137 & 2.137 & 10.26 & 0.265 & 0.266 & 0.266 & 0.264 & 1.045 & 1.084 & 1.084 & 1.086\\
&  & m & 78.58 & 0.505 & 0.505 & 0.525 & 78.50 & 0.457 & 0.457 & 0.459 & 0.257 & 0.260 & 0.260 & 0.259 & 0.999 & 1.073 & 1.073 & 1.063\\


\bottomrule
\end{tabular}
\end{table}

==> Ranks.tex <==
\begin{table}
 \centering
\caption{Ranking of the methods according to the MSE values}
\label{tab5}
\begin{tabular}{cccccccccc}
\toprule
GLD Setting & n & pdQ & TL & PM & ML & MPS & TM & SM & DLA\\
\midrule
gld(0,1,1.5,1.5) & 100 & 3 & 7 & 8 & 4 & 1 & 2 & 5 & 5\\
& 250 & 1 & 7 & 8 & 5 & 1 & 3 & 4 & 6\\
& 500 & 1 & 5 & 8 & 7 & 3 & 2 & 4 & 5\\
& 1000 & 1 & 6 & 8 & 7 & 4 & 5 & 2 & 3\\
\midrule
gld(0,1,2.5,1.5) & 100 & 2 & 7 & 8 & 4 & 2 & 1 & 5 & 5\\
& 250 & 1 & 7 & 8 & 6 & 2 & 4 & 5 & 2\\
& 500 & 1 & 8 & 5 & 7 & 3 & 4 & 5 & 2\\
& 1000 & 1 & 7 & 4 & 8 & 3 & 5 & 6 & 2\\
\midrule
gld(0,1,2,0.5) & 100 & 5 & 3 & 8 & 7 & 2 & 1 & 6 & 4\\
& 250 & 1 & 2 & 8 & 7 & 3 & 4 & 5 & 6\\
& 500 & 5 & 2 & 7 & 8 & 2 & 1 & 2 & 6\\
& 1000 & 5 & 4 & 6 & 8 & 1 & 2 & 3 & 6\\
\midrule
gld(0,1,0.5,0.6) & 100 & 6 & 3 & 8 & 5 & 2 & 1 & 4 & 7\\
& 250 & 6 & 5 & 8 & 3 & 1 & 1 & 4 & 7\\
& 500 & 6 & 5 & 8 & 3 & 1 & 1 & 4 & 7\\
& 1000 & 5 & 5 & 8 & 1 & 1 & 1 & 4 & 7\\
\bottomrule
\end{tabular}
\end{table}

==> tab0133.tex <==
\begin{table}[h]
\tiny
  \centering
  
    \caption{This table shows a comparison of the mean standard error and the absolute bias of the GLD parameters represented by $\lambda_1$,$\lambda_2$,$\lambda_3$ and $\lambda_4$ between several fitting methods.The considered methods are Method of Probability Density Quantiles(pdQ), Method of TL-moments (TL), Percentile Matching Method (PM,) Numerical Maximum Likelihood (ML), Maximum Product of Spacings (MPS), Titterington's Method (TM), Starship Method (SM), and Method of Distributional Least Absolutes (DLA). These values are calculated for 500 fitting results for actual parameters $\lambda_1=0$, $\lambda_2=1$, $\lambda_3=3$ and $\lambda_4=3$  }
\label{tab5}
\hspace*{-0.5cm}

\begin{tabular}{lrlllllllll}
\toprule
n & Est & pdQ & TL & PM & ML & MPS & TM & SM & DLA\\
%50 & l1 & 0.002  (0.001) & 0.002  (0.001) & 0.003  (0.002) & 0.002  (0.001) & 0.002  (0.001) & 0.002  (0.001) & 0.002  (0.001) & 0.002  (0.001)\\
%& l2 & 14.233  (3.353) & 24.176  (4.533) & 50.271  (5.688) & 9.900  (2.899) & 18.067  (3.777) & 19.289  (3.928) & 30.656  (4.907) & 20.814  (4.089)\\
% & l3 & 4.790  (2.150) & 6.037  (2.433) & 6.280  (2.418) & 4.560  (2.120) & 5.379  (2.275) & 5.693  (2.261) & 6.236  (2.464) & 5.496  (2.298)\\
 %& l4 & 4.829  (2.148) & 6.068  (2.438) & 6.352  (2.433) & 4.586  (2.125) & 5.401  (2.279) & 5.436  (2.283) & 6.248  (2.467) & 5.534  (2.300)\\
\midrule
100 & l1 & 0.001  (0.002) & 0.001  (0.002) & 0.001  (0.001) & 0.001  (0.001) & 0.001  (0.002) & 0.001  (0.002) & 0.001  (0.002) & 0.001  (0.002)\\
 & l2 & 15.613  (3.762) & 20.756  (4.411) & 34.255  (5.231) & 8.882  (2.867) & 13.615  (3.535) & 14.013  (3.595) & 21.100  (4.405) & 18.361  (4.081)\\
 & l3 & 5.205  (2.269) & 6.215  (2.487) & 6.573  (2.518) & 4.763  (2.175) & 5.450  (2.325) & 5.452  (2.326) & 6.170  (2.474) & 5.835  (2.390)\\
 & l4 & 5.138  (2.250) & 6.154  (2.472) & 6.520  (2.507) & 4.723  (2.165) & 5.391  (2.308) & 5.399  (2.311) & 6.113  (2.459) & 5.755  (2.369)\\
 \midrule
 
250 & l1 & 0.000  (0.001) & 0.000  (0.002) & 0.000  (0.002) & 0.000  (0.001) & 0.000  (0.001) & 0.000  (0.001) & 0.000  (0.002) & 0.000  (0.001)\\
 & l2 & 14.098  (3.678) & 19.801  (4.380) & 30.273  (5.218) & 9.490  (3.029) & 12.022  (3.419) & 12.159  (3.439) & 18.739  (4.246) & 18.684  (4.246)\\
 & l3 & 5.228  (2.282) & 6.252  (2.497) & 6.899  (2.611) & 5.025  (2.238) & 5.419  (2.325) & 5.415  (2.324) & 6.130  (2.472) & 6.121  (2.468)\\
 & l4 & 5.211  (2.278) & 6.199  (2.487) & 6.842  (2.599) & 4.992  (2.231) & 5.384  (2.318) & 5.380  (2.317) & 6.075  (2.461) & 6.076  (2.461)\\

\midrule
500 & l1 & 0.000  (0.001) & 0.000  (0.000) & 0.000  (0.000) & 0.000  (0.001) & 0.000  (0.000) & 0.000  (0.000) & 0.000  (0.000) & 0.000  (0.000)\\
 & l2 & 13.937  (3.697) & 18.984  (4.326) & 27.092  (5.090) & 9.747  (3.097) & 11.216  (3.326) & 11.273  (3.333) & 17.331  (4.129) & 18.396  (4.256)\\
 & l3 & 5.343  (2.309) & 6.218  (2.492) & 6.912  (2.622) & 5.115  (2.260) & 5.341  (2.310) & 5.331  (2.305) & 6.044  (2.457) & 6.164  (2.481)\\
 & l4 & 5.319  (2.304) & 6.217  (2.492) & 6.913  (2.623) & 5.105  (2.258) & 5.332  (2.308) & 5.326  (2.306) & 6.042  (2.457) & 6.160  (2.480)\\
\midrule
1000 & l1 & 0.000  (0.001) & 0.000  (0.001) & 0.000  (0.001) & 0.000  (0.001) & 0.000  (0.000) & 0.000  (0.000) & 0.000  (0.000) & 0.000  (0.001) & 0.000  (0.001)\\
 & l2 & 14.367  (3.773) & 14.367  (3.773) & 18.824  (4.322) & 26.421  (5.079) & 9.777  (3.117) & 10.670  (3.257) & 10.701  (3.262) & 16.972  (4.102) & 18.647  (4.299)\\
 & l3 & 5.460  (2.336) & 5.460  (2.336) & 6.241  (2.497) & 6.977  (2.638) & 5.153  (2.269) & 5.287  (2.299) & 5.286  (2.299) & 6.045  (2.458) & 6.232  (2.496)\\
 & l4 & 5.452  (2.334) & 5.452  (2.334) & 6.218  (2.493) & 6.939  (2.631) & 5.149  (2.269) & 5.285  (2.299) & 5.284  (2.298) & 6.026  (2.454) & 6.208  (2.491)\\
\bottomrule

\end{tabular}
\end{table}
